Structures on the Category of N-Complexes

The theory of $N$-complexes is a generalization of both ordinary chain complexes and graded objects. Hence it yields deeper insight in the structure of these and offers a broader range of applications. This work generalizes the tensor product of chain complexes and graded objects to the case of $N$-complexes using the structures of $q$-binomial coefficients. We then study different approaches to realize the derived category of $N$-complexes. In particular we realize it as the Verdier quotient of the homotopy category of $N$-complexes, as the $\mathrm{h}$-projective objects and as the homotopy category of a category admitting a Quillen model structure.

==> Category_KN.tex <==
\section{$N$-complexes in semisimple categories}




In this section we will show that the homotopy category and the derived category coincide if $\A$ is semisimple, i.\,e.\ a category such that every short exact sequence splits.



\begin{proposition}\label{6.4}
Let $X \in \CC_N(\A)$, where $\A$ is a semisimple abelian category and $N \in \N$. Then 
$X=0$ in $\KK_N(\A)$ if and only if  $H^*_{(r)}(X)=0$ $\forall r \in \{ 1,...,N-1\}$.

\begin{proof} $\;$
\begin{enumerate}
\item[''$\Rightarrow$'':]This implication is just Lemma~\ref{5.6} applied to the identity combined with Proposition~\ref{5.4}.
\item[''$\Leftarrow$'':]
Throughout this proof the following diagram will be important: 
\begin{equation*}
\tikz[heighttwo,xscale=2.8,yscale=2,baseline]{

 \node (ker1) at (0,0){$\ker(d)^n$};
 \node (ker2) at (1,0){$\ker(d^2)^n$};
 \node (ker3) at (2,0){$\ker(d^3)^n$};
\node (P1) at (3,0){$\cdot \cdot \cdot$}; 
\node (P2) at (3,1){$\cdot \cdot \cdot$}; 

   \node (kerN) at (4.2,0){$\ker(d^{N-1})^n$};
    \node (Xn) at (5.2,0){$X^n$};
    
    
    
     \node (ker2_1) at (0,1){$\ker(d)^{n+1}$};
 \node (ker2_2) at (1,1){$\ker(d^2)^{n+1}$};
 \node (ker2_3) at (2,1){$\ker(d^3)^{n+1}$};
 
 
   \node (ker2_N) at (4.2,1){$\ker(d^{N-1})^{n+1}$};
    \node (Xn+1) at (5.2,1){$X^{n+1}$};

\draw[->]
(ker2) edge node[above] {$d$} (ker2_1)
(ker3) edge node[above] {$d$} (ker2_2)
(P1) edge node[above] {$d$} (ker2_3)
(kerN) edge node[above] {$d$} (P2)
(Xn) edge node[above] {$d$} (ker2_N)
;


\draw[right hook->](ker1)to(ker2);
\draw[right hook->](ker2)to(ker3);
\draw[right hook->](ker3)to(P1);

\draw[right hook->](P1)to(kerN);

\draw[right hook->](kerN)to(Xn);

\draw[right hook->](ker2_1)to(ker2_2);
\draw[right hook->](ker2_2)to(ker2_3);
\draw[right hook->](ker2_3)to(P2);

\draw[right hook->](P2)to(ker2_N);

\draw[right hook->](ker2_N)to(Xn+1);


}.
\end{equation*}
Since $H^*_{(r)}(X)=0$ $\forall r \in \{1,...,N-1\}$, it follows that $\ker(d^r)^n=\im(d^{N-r})^n$ and hence \\ $d^{N-r}:X^{n-N+r} \twoheadrightarrow  \ker(d^r)^n$ is an epimorphism and so is $d: \ker (d^{r+1})^n \twoheadrightarrow \ker (d^r)^{n+1}$:
\begin{equation*}
\tikz[heighttwo,xscale=2.8,yscale=2,baseline]{

 \node (ker1) at (0,0){$\ker(d)^n$};
 \node (ker2) at (1,0){$\ker(d^2)^n$};
 \node (ker3) at (2,0){$\ker(d^3)^n$};
\node (P1) at (3,0){$\cdot \cdot \cdot$}; 
\node (P2) at (3,1){$\cdot \cdot \cdot$}; 

  \node (kerN) at (4.2,0){$\ker(d^{N-1})^n$};
    \node (Xn) at (5.2,0){$X^n$};
    
    
    
     \node (ker2_1) at (0,1){$\ker(d)^{n+1}$};
 \node (ker2_2) at (1,1){$\ker(d^2)^{n+1}$};
 \node (ker2_3) at (2,1){$\ker(d^3)^{n+1}$};
 
 \node (ker2_N) at (4.2,1){$\ker(d^{N-1})^{n+1}$};
    \node (Xn+1) at (5.2,1){$X^{n+1}$};
    
\draw[->>]
(ker2) edge node[above] {$d$} (ker2_1)
(ker3) edge node[above] {$d$} (ker2_2)
(P1) edge node[above] {$d$} (ker2_3)
(kerN) edge node[above] {$d$} (P2)
(Xn) edge node[above] {$d$} (ker2_N)
;


\draw[right hook->](ker1)to(ker2);
\draw[right hook->](ker2)to(ker3);
\draw[right hook->](ker3)to(P1);

\draw[right hook->](P1)to(kerN);
\draw[right hook->](kerN)to(Xn);

\draw[right hook->](ker2_1)to(ker2_2);
\draw[right hook->](ker2_2)to(ker2_3);
\draw[right hook->](ker2_3)to(P2);

\draw[right hook->](P2)to(ker2_N);
\draw[right hook->](ker2_N)to(Xn+1);


}.
\end{equation*}
Since $d: \ker (d^{r+1})^n \twoheadrightarrow \ker (d^r)^{n+1}$ is an epimorphism in the semisimple category $\A$, it splits. So there are sections
\begin{equation*}
s^i_n:\ker(d^i)^n\to \ker (d^{i-1})^{n+1}
\end{equation*}
and $\ker(d^j)^n= \ker(d^{j-1})^{n+1}\oplus \ker(d)^n$. So inductively 
\begin{equation*}
X^n \cong \ker(d)^n \oplus \ker(d)^{n+1} \oplus ... \oplus \ker(d)^{n+N-2} \oplus \ker(d)^{n+N-1}.
\end{equation*}In the diagram these $s_n^i$ look like:

\begin{equation*}
\tikz[heighttwo,xscale=2.8,yscale=2,baseline]{

\node (ker1) at (0,0){$\ker(d)^n$};
 \node (ker2) at (1,0){$\ker(d^2)^n$};
 \node (ker3) at (2,0){$\ker(d^3)^n$};
\node (P1) at (3,0){$\cdot \cdot \cdot$}; 
\node (P2) at (3,1){$\cdot \cdot \cdot$}; 

   \node (kerN) at (4.2,0){$\ker(d^{N-1})^n$};
    \node (Xn) at (5.2,0){$X^n$};
    
    
    
     \node (ker2_1) at (0,1){$\ker(d)^{n+1}$};
 \node (ker2_2) at (1,1){$\ker(d^2)^{n+1}$};
 \node (ker2_3) at (2,1){$\ker(d^3)^{n+1}$};
 
 \node (ker2_N) at (4.2,1){$\ker(d^{N-1})^{n+1}$};
    \node (Xn+1) at (5.2,1){$X^{n+1}$};

\draw[->>]
(ker2) edge node[above] {$d$} (ker2_1)
(ker3) edge node[above] {$d$} (ker2_2)
(P1) edge node[above] {$d$} (ker2_3)
(kerN) edge node[above] {$d$} (P2)
(Xn) edge node[above] {$d$} (ker2_N)
;

\draw[dashed, ->]
(ker2_1) edge [bend right=30] node[left] {\small{$s^{n+1}_1$}} (ker2)
(ker2_2) edge[bend right=30] node[left] {$s^{n+1}_2$} (ker3)
(ker2_3) edge[bend right=30] node[left] {$s^{n+1}_3$} (P1)
(P2) edge[bend right=30] node[left] {$s^{n+1}_{N-3}$} (kerN)
(ker2_N) edge[bend right=30] node[left] {$s^{n+1}_{N-1}$} (Xn)
;

\draw[right hook->](ker1)to(ker2);
\draw[right hook->](ker2)to(ker3);
\draw[right hook->](ker3)to(P1);

\draw[right hook->](P1)to(kerN);
\draw[right hook->](kerN)to(Xn);

\draw[right hook->](ker2_1)to(ker2_2);
\draw[right hook->](ker2_2)to(ker2_3);
\draw[right hook->](ker2_3)to(P2);

\draw[right hook->](P2)to(ker2_N);
\draw[right hook->](ker2_N)to(Xn+1);

}.
\end{equation*}
Define $\widehat{s}^i:=s^{i-N+1}_{N-1}\circ s^{i-N+2}_{N-2}...\circ s^{i-1}_2\circ s^i_1:\ker(d)^{i-N+1} \to X^{i-N+1}$. By the above decomposition of $X^i$ as direct sum, these $\widehat{s}^i$ now induce a map $s:X^i \to X^{i-N+1}$ by setting $s=0$ on all other summands. These $s^i$ now fulfil 
\begin{equation*}
\id_{X^i}=\sum_{j=1}^{N-1}  d^{N-j}s^{i+j-1}d^{j-1},
\end{equation*}
since $d^{N-j}s^{i+j-1}d^{j-1}(x)\neq 0$ if and only if $d^j(x)=0$, and $d^{j-1}\neq 0$ and
in this case this yields:
\begin{equation*}
d^{N-j}s^{i+j-1}d^{j-1}(x)=x.\qedhere
\end{equation*}
\end{enumerate}
\end{proof}
\end{proposition}

\begin{remark}\label{acyclic nullhomotopic}Regarding the previous proposition there are two remarks to be made:
\begin{enumerate}
\item A natural example for $\A$ is the category of vector spaces over a field.
\item It is very essential for this proof that $\A$ is semisimple. Let for example  $\A$ be the category $\Mod_\Z$. Then this theorem does not hold. For example the $N$-complex

\begin{equation*}
\tikz[heighttwo,xscale=2,yscale=2,baseline]{

\node (P0) at (0,0){$\cdot \cdot \cdot$};
\node (X1) at (1,0){$\Z/(p^N)$};
\node (X2) at (2,0){$\Z/(p^N)$};
\node (X3) at (3,0){$\Z/(p^N)$};
\node (P1) at (4,0){$\Z/(p^N)$}; 
\node (XN-2) at (5,0){$\Z/(p^N)$};
\node (P2) at (6,0){$\cdot \cdot \cdot$};
    
\draw[->]
(P0) edge node[above] {$p$} (X1)
(X1) edge node[above] {$p$} (X2)
(X2) edge node[above] {$p$} (X3)
(X3) edge node[above] {$p$} (P1)
(P1) edge node[above] {$p$} (XN-2)
(XN-2) edge node[above] {$p$} (P2);
}
\end{equation*}
with $0 \neq p \in \Z$ has trivial cohomology as an $N$-complex of $\Z$-modules, but it is not nullhomotopic, since if it would be nullhomotopic the following must hold:
\begin{equation*}
1=\sum_{j=1}^{N-1} d^{N-j}s^{i+j-1}d^{j-1}(1)=\sum_{j=1}^{N-1} p^{N-j}s^{i+j-1}p^{j-1}(1)=p^{N-1}\sum_{j=1}^{N-1} s^{i+j-1}(1).
\end{equation*}
But this would mean that there exists an element $x\in \Z/p^N\Z$ such that $xp^{N-1}=1$, which is a contradiction if $p \neq \pm 1$ and $1<N$.
\end{enumerate} 
\end{remark}

 \begin{corollary}
 Let $\kk$ be a field, and $X \in \CC_N(\Mod_\kk)$. Then $X$ is nullhomotopic if and only if $ X \cong \bigoplus _{i \in \mathbb{Z}} \mu_N^i ({\kk^{\oplus I_i}})$.
\begin{proof}
This is clear by the proof of Proposition~\ref{6.4}, since $\Mod_\kk$ is semisimple and every $\kk$-module $X$ is isomorphic to $\kk^{\oplus I_X}$.
\end{proof}
\end{corollary}


\begin{corollary}\label{6.6}

Let $\A$ be a semisimple category, $N \in \N$ and $f:X \to Y$. Then $f$ is an isomorphism in $\KK_N(\A)$ if and only if $f$ is an $N$-quasi-isomorphism.

\begin{proof}
By the definition of $\KK_N(\A)$ a morphism in $\KK_N(\A)$ is an isomorphism if and only if $\Cone_{\KK_N(\A)}(f)\cong 0$. Furthermore $f$ is by Corollary~\ref{5.9} an $N$-quasi-isomorphism precisely if $H^i_{(r)}(\Cone_{\KK_N(\A)}(f))=0$ for all $ r \in \{ 1,...,N-1\}$ and $i \in \Z$. But by Theorem~\ref{6.4} these two statements are equivalent. 
%But this is clear from the previous proposition. (It is important to note here that the cone conventions from \cite{N-complex}  coincide for $K_N(\Mod_k)$ and $D_N(\Mod_k)$) 
\end{proof}
\end{corollary}



\newpage

==> N-Bar-construction.tex <==
\section{N-Bar-construction}

\begin{definition}
Let $A$ be an associative algebra over a field $k$ and $N \in \N$ such that there exists an $N$-root of unity $\xi \neq 1$. 
\begin{enumerate}
\item Define for all $n\in \N$ and $i <n$ the map $d_{n,i}:A^{\otimes n+1} \to A^{\otimes n}$ as the map defined by 
\begin{align*} 
d_{n,i}(a_0 \otimes a_1\otimes...\otimes a_{n})=a_0 \otimes a_1\otimes...a_{i-1}\otimes a_i a_{i+1} \otimes a_{i+2}\otimes...\otimes a_{n}.
\end{align*}
\item Define the complex $C'_N(A)$ as the $\infty$-complex:
\begin{equation*}
\tikz[heighttwo,xscale=2,yscale=2,baseline]{

\node (P0) at (0,0){$\cdot \cdot \cdot$};
\node (X1) at (-1,0){$0$};
\node (X2) at (-2,0){$A$};
\node (X3) at (-3,0){$A^{\otimes2}$};
\node (X4) at (-4,0){$A^{\otimes3}$};
\node (X5) at (-5,0){$A^{\otimes4}$};

\node (P2) at (-6,0){$\cdot \cdot \cdot$};
    
\node (P3) at (0,0.5){$\cdot \cdot \cdot$};
\node (i-n-1) at (-1,0.5){\tiny{ $1$}};
\node (i-n) at (-2,0.5){\tiny{$0$}};
\node (i-n+1) at (-3,0.5){\tiny{$-1$}};
\node (P4) at (-4,0.5){\tiny{$-2$}};
\node (i-1) at (-5,0.5){\tiny{$-3$}};
\node (i) at (-6,0.5){\tiny{$\cdot \cdot \cdot$}};

    
\draw[->]
(X2) edge node[above] {$0$} (X1)
(X1) edge node[above] {$0$} (P0)
(X3) edge node[above] {$b_0$} (X2)
(X4) edge node[above] {$b_1$} (X3)
(X5) edge node[above] {$b_2$} (X4)
(P2) edge node[above] {$b_3$} (X5);
}
\end{equation*}
where $b_{j}:A^{\otimes j+2} \to A^{\otimes j+1}$ is defined by 
\begin{align*}b_j(a_0 \otimes a_1\otimes...\otimes a_{j+1})=\sum_{i=0}^{j} \xi^i d_{j+1,i}(a_0 \otimes a_1\otimes...\otimes a_{j+1})
\end{align*}
\end{enumerate}
\end{definition}
\begin{Huge}
TBD
\end{Huge}

==> NdgMod.tex <==

\section{The category of N-dg-A modules}
\begin{definition}
Let $\A$ be an abelian category, and $N\in \N$.
\begin{enumerate}
\item
A $N$-dg-$A$-module is a pair $(X,d_X)$ where $X$ is a graded $A$-module and $d_X:X\to X$ is a $N$-differential, that is a degree $1$ morphism of graded modules such that the equation 
\begin{equation*}
d_X^N=0
\end{equation*}
holds. abusing the notation we often identify $(X,d_X)$ with its underlying graded module $X$.
\item
Let $(X,d_X)$ and $(Y,d_y)$ be two $N$-dg-$A$-modules. A morphism of $N$-dg-$A$-modules $f:(X,d_X)\to (Y,d_Y)$ is a morphism of graded $A$-modules $f:X \to Y$ for which the equation
\begin{equation*}
d_Y\circ f = f \circ d_X
\end{equation*}
\item
Define $\NdgMod_A$ as the category whose objects are $N$-dg-$A$-modules and whose morphisms are morphisms of $N$-dg-$A$-modules.
\end{enumerate}
\end{definition}

\begin{proposition}
The category $\NdgMod_A$ is a complete and cocomplete abelian category.
\begin{proof}
\begin{enumerate}
\item[pointed]
The category $\NdgMod_A$ is pointed with $(0,0)$ being the zero object, since the equation
\begin{equation*}
 d_X \circ 0=0=0 \circ 0
\end{equation*}
holds for all $(X,d_X)\in \NdgMod_A$
\item[cokernels]
Let $f:X \to Y$ be a morphism of $N$-dg-$A$-modules and let $g:Y \to Z$ be its cokernel in $\grMod_A$. We want to exhibit  $Z$ with a differential such that $g$ becomes a cokernel of $f$ in $\NdgMod_A$.
To that end observe that by the universal property of $g$ the dashed arrow in the following diagram in $grMod_A$ can be filled:
\begin{equation*}
\tikz[heighttwo,xscale=2.3,yscale=2,baseline]{

\node (X1) at (0,1){$X$};
\node (X2) at (0,0){$X$};
\node (Y1) at (1,1){$Y$};
\node (Y2) at (1,0){$Y$};
\node (Z1) at (2,1){$Z$};
\node (Z2) at (2,0){$Z$};

\draw[->]
(X1) edge node[right] {$d_X$} (X2)
(Y1) edge node[right] {$d_Y$} (Y2)

(X1) edge node[above] {$f$} (Y1)
(Y1) edge node[above] {$g$} (Z1)

(X2) edge node[above] {$f$} (Y2)
(Y2) edge node[above] {$g$} (Z2)
;
\draw[dashed,->]
(Z1) edge node[right] {$d_Z$} (Z2);
}.
\end{equation*}
This is now our candidate for $d_Z$, so it just remains to prove that $(d_Z)^N=0$, but this is true by the commutativity of the following diagram:

\begin{equation*}
\tikz[heighttwo,xscale=2.3,yscale=2,baseline]{

\node (X1) at (0,1){$X$};
\node (X2) at (0,0){$X$};
\node (Y1) at (1,1){$Y$};
\node (Y2) at (1,0){$Y$};
\node (Z1) at (2,1){$Z$};
\node (Z2) at (2,0){$Z$};

\node (P1) at (1,-0.4){$\cdot$};
\node (P2) at (1,-0.5){$\cdot$};
\node (P3) at (1,-0.6){$\cdot$};

\node (XN-1) at (0,-1){$X$};
\node (XN) at (0,-2){$X$};
\node (YN-1) at (1,-1){$Y$};
\node (YN) at (1,-2){$Y$};
\node (ZN-1) at (2,-1){$Z$};
\node (ZN) at (2,-2){$Z$};

\draw[->]
(X1) edge node[right] {$d_X$} (X2)
(Y1) edge node[right] {$d_Y$} (Y2)
(Z1) edge node[right] {$d_Z$} (Z2)


(XN-1) edge node[right] {$d_X$} (XN)
(YN-1) edge node[right] {$d_Y$} (YN)
(ZN-1) edge node[right] {$d_Z$} (ZN)


(X1) edge node[above] {$f$} (Y1)
(Y1) edge node[above] {$g$} (Z1)

(X2) edge node[above] {$f$} (Y2)
(Y2) edge node[above] {$g$} (Z2)

(XN-1) edge node[above] {$f$} (YN-1)
(YN-1) edge node[above] {$g$} (ZN-1)

(XN) edge node[above] {$f$} (YN)
(YN) edge node[above] {$g$} (ZN)

(Y1) edge [bend right=25] node[left] {$(d_Y)^N=0$} (YN)
(Z1) edge [bend left=25] node[right] {$(d_Z)^N=0$} (ZN)
;
}.
\end{equation*}
Hence $(Z,d_Z)$ is a cokernel for $f$ in $\NdgMod_A$.
\item{kernels}
Let $g:Y \to Z$ be a morphism of $N$-dg-$A$-modules and let $f:X\to Y$ be its kernel in $\grMod_A$. We want to exhibit again $X$ with a differential such that $f$ becomes the kernel in $\NdgMod_A$.
To that end observe that by the universal property of $g$ the dashed arrow in the following diagram in $grMod_A$ can be filled:
\begin{equation*}
\tikz[heighttwo,xscale=2.3,yscale=2,baseline]{

\node (X1) at (0,1){$X$};
\node (X2) at (0,0){$X$};
\node (Y1) at (1,1){$Y$};
\node (Y2) at (1,0){$Y$};
\node (Z1) at (2,1){$Z$};
\node (Z2) at (2,0){$Z$};

\draw[->]
(Z1) edge node[right] {$d_Z$} (Z2)
(Y1) edge node[right] {$d_Y$} (Y2)

(X1) edge node[above] {$f$} (Y1)
(Y1) edge node[above] {$g$} (Z1)

(X2) edge node[above] {$f$} (Y2)
(Y2) edge node[above] {$g$} (Z2)
;
\draw[dashed,->]
(X1) edge node[right] {$d_X$} (X2);
}.
\end{equation*}
This is now our candidate for $d_X$, so it just remains to prove that $(d_X)^N=0$, but this is true by the commutativity of the following diagram:

\begin{equation*}
\tikz[heighttwo,xscale=2.3,yscale=2,baseline]{

\node (X1) at (0,1){$X$};
\node (X2) at (0,0){$X$};
\node (Y1) at (1,1){$Y$};
\node (Y2) at (1,0){$Y$};
\node (Z1) at (2,1){$Z$};
\node (Z2) at (2,0){$Z$};

\node (P1) at (1,-0.4){$\cdot$};
\node (P2) at (1,-0.5){$\cdot$};
\node (P3) at (1,-0.6){$\cdot$};

\node (XN-1) at (0,-1){$X$};
\node (XN) at (0,-2){$X$};
\node (YN-1) at (1,-1){$Y$};
\node (YN) at (1,-2){$Y$};
\node (ZN-1) at (2,-1){$Z$};
\node (ZN) at (2,-2){$Z$};

\draw[->]
(X1) edge node[right] {$d_X$} (X2)
(Y1) edge node[right] {$d_Y$} (Y2)
(Z1) edge node[right] {$d_Z$} (Z2)


(XN-1) edge node[right] {$d_X$} (XN)
(YN-1) edge node[right] {$d_Y$} (YN)
(ZN-1) edge node[right] {$d_Z$} (ZN)


(X1) edge node[above] {$f$} (Y1)
(Y1) edge node[above] {$g$} (Z1)

(X2) edge node[above] {$f$} (Y2)
(Y2) edge node[above] {$g$} (Z2)

(XN-1) edge node[above] {$f$} (YN-1)
(YN-1) edge node[above] {$g$} (ZN-1)

(XN) edge node[above] {$f$} (YN)
(YN) edge node[above] {$g$} (ZN)

(X1) edge [bend right=25] node[left] {$(d_X)^N=0$} (XN)
(Y1) edge [bend left=25] node[right] {$(d_Y)^N=0$} (YN)
;
}.
\end{equation*}
\item[monos are the cokernels of their kernels]
Since kernels and cokernels are induced by the cokernels and kernels in $\grMod_A$ this property is clear, since $\grMod_A$ is abelian.
\item[direct sums]
This follows immediately once we showed completeness and cocompleteness, since $(X,d_X) \oplus (Y,d_Y)$ is just the pushout:
\begin{equation*}
\tikz[heighttwo,xscale=2.3,yscale=-2,baseline]{

\node (0) at (0,0){$0$};
\node (X) at (1,0){$X$};
\node (Y) at (0,1){$Y$};
\node (X+Y) at (1,1){$X \oplus Y$};

\draw[->]
(0) edge node[right] {} (X)
(0) edge node[right] {} (Y)

(X) edge node[above] {} (X+Y)
(Y) edge node[above] {} (X+Y);
}.
\end{equation*}
\item[complete]
Let $I$ be a be a small category, we want to show that there exists a limit over $I$ of $(X_i,d_{X_i}$. Hence let  $\widehat{\lim_{i\in I} X_i }$ be the Limit over $I$ of $X_i$ regarded in $\grMod_A$. We want to show that this already defines a $N$-dg-$A$-module. For this consider for all $i \in I$ the following diagram:
\begin{equation*}
\tikz[heighttwo,xscale=5,yscale=-2,baseline]{

\node (P1) at (0,0){$\widehat{\lim_{i\in I} X_i }$};
\node (P2) at (1,0){$\widehat{\lim_{i\in I} X_i }$};
\node (X1) at (0,1){$ X_i$};
\node (X2) at (1,1){$X_i$};

\draw[->]
(P1) edge node[left] {$\pi_i$} (X1)

(P2) edge node[right] {$\pi_i$} (X2)
(X1) edge node[above] {$d_{X_i}$} (X2);
\draw[dashed,->]
(P1) edge node[below] {$d_{\widehat{\lim_{i\in I} X_i }}$} (P2);
}.
\end{equation*}
Now since all the structure maps have to be in $\NdgMod_A$ they commute with $d_{X_i}$ and hence the maps $d_{X_i}\circ \pi$ define a morphism of diagrams in $\grMod_A$ and so the dottted arrow can be filled.

This is now our candidate for the differential. And indeed by the commutative diagram

\begin{equation*}
\tikz[heighttwo,xscale=5,yscale=-2,baseline]{

\node (P1) at (0,0){$\widehat{\lim_{ I} X_i }$};
\node (P2) at (1,0){$\widehat{\lim_{ I} X_i }$};
\node (X1) at (0,1){$ X_i$};
\node (X2) at (1,1){$X_i$};

\node (PN-1) at (2,0){$\widehat{\lim_{ I} X_i }$};
\node (PN) at (3,0){$\widehat{\lim_{I} X_i }$};
\node (XN-1) at (2,1){$ X_i$};
\node (XN) at (3,1){$X_i$};

\node (pt) at (1.5,0.5){$ \cdots$};
\node (pt1) at (1.25,1){};
\node (pt2) at (1.25,0){};
\node (pt3) at (1.75,0){};
\node (pt4) at (1.75,1){};




\draw[->]
(P1) edge node[left] {$\pi_i$} (X1)
(P1) edge node[below] {$d_{\widehat{\lim_{ I} X_i }}$} (P2)
(P2) edge node[right] {$\pi_i$} (X2)
(X1) edge node[above] {$d_{X_i}$} (X2)

(PN-1) edge node[left] {$\pi_i$} (XN-1)
(PN-1) edge node[below] {$d_{\widehat{\lim_{I} X_i }}$} (PN)
(PN) edge node[right] {$\pi_i$} (XN)
(XN-1) edge node[above] {$d_{X_i}$} (XN)

(P2) edge (pt2)
(X2) edge (pt1)
(pt3) edge (PN-1)
(pt4) edge (XN-1)

(X1) edge [bend left=25] node[below] {$(d_{X_i})^N=0$} (XN)



;





\draw[dashed,->]
;
}.
\end{equation*}

it fulfils 
\begin{equation*}
(d_{\widehat{\lim_{i\in I} X_i }})^N=0
\end{equation*} 
\item[cocompleteness]
Let $I$ be a small category, again we want to show that there exists the colimit of $(X_i,d_{X_i})$ over $I$. For this again consider the colimit $\widehat{colim_I X_i}$ in $\grMod_A$. This we will now equip with an $N$ differential, for this consider the commutative diagram:
\begin{equation*}
\tikz[heighttwo,xscale=5,yscale=-2,baseline]{

\node (P1) at (0,1){$\widehat{\lim_{i\in I} X_i }$};
\node (P2) at (1,1){$\widehat{\lim_{i\in I} X_i }$};
\node (X1) at (0,0){$ X_i$};
\node (X2) at (1,0){$X_i$};

\draw[->]
(X1) edge node[left] {$\iota_i$} (P1)

(X2) edge node[right] {$\iota_i$} (P2)
(X1) edge node[above] {$d_{X_i}$} (X2);
\draw[dashed,->]
(P1) edge node[below] {$d_{\widehat{\lim_{i\in I} X_i }}$} (P2);
}.
\end{equation*}
Here the $d_{X_i}$ comute with all morphisms in the diagram by the fact that they are $N$-dg-$A$-morphisms, and hence they define a morphism of diagrams, and so by the definition of th colimit the dashed arrow can be filled.
This will be again our candidate for a $N$-differential. Now to show that this actually defines an $N$-differential consider the following commutative diagram:
\begin{equation*}
\tikz[heighttwo,xscale=5,yscale=-2,baseline]{

\node (P1) at (0,1){$\widehat{\lim_{ I} X_i }$};
\node (P2) at (1,1){$\widehat{\lim_{ I} X_i }$};
\node (X1) at (0,0){$ X_i$};
\node (X2) at (1,0){$X_i$};

\node (PN-1) at (2,1){$\widehat{\lim_{ I} X_i }$};
\node (PN) at (3,1){$\widehat{\lim_{I} X_i }$};
\node (XN-1) at (2,0){$ X_i$};
\node (XN) at (3,0){$X_i$};

\node (pt) at (1.5,0.5){$ \cdots$};
\node (pt1) at (1.25,1){};
\node (pt2) at (1.25,0){};
\node (pt3) at (1.75,0){};
\node (pt4) at (1.75,1){};




\draw[->]
(P1) edge node[left] {$\iota_i$} (X1)
(P1) edge node[below] {$d_{\widehat{\lim_{ I} X_i }}$} (P2)
(P2) edge node[right] {$\iota_i$} (X2)
(X1) edge node[below] {$d_{X_i}$} (X2)

(PN-1) edge node[left] {$\iota_i$} (XN-1)
(PN-1) edge node[below] {$d_{\widehat{\lim_{I} X_i }}$} (PN)
(PN) edge node[right] {$\iota_i$} (XN)
(XN-1) edge node[below] {$d_{X_i}$} (XN)

(P2) edge (pt1)
(X2) edge (pt2)
(pt4) edge (PN-1)
(pt3) edge (XN-1)

(X1) edge [bend right=25] node[above] {$(d_{X_i})^N=0$} (XN)
;

}.
\end{equation*}
\end{enumerate}
\end{proof}
\end{proposition}

\begin{proposition}
The split short exact sequences in $\NdgMod_A$ define an exact structure
\begin{proof}
the split short exact sequences define anexact structure on $\grMod_A$. Now, since all limits and colimits are as objects computed in $\grMod_A$, this also defines an exact structure on $\NdgMod_A$.
\end{proof}
\end{proposition}

\begin{definition}
We call the exact structure of the split short exact sequences $\So$
\end{definition}


